Batch Ensemble for Variance Dependent Regret in Stochastic Bandits

Efficiently trading off exploration and exploitation is one of the key challenges in online Reinforcement Learning (RL). Most works achieve this by carefully estimating the model uncertainty and following the so-called optimistic model. Inspired by practical ensemble methods, in this work we propose a simple and novel batch ensemble scheme that provably achieves near-optimal regret for stochastic Multi-Armed Bandits (MAB). Crucially, our algorithm has just a single parameter, namely the number of batches, and its value does not depend on distributional properties such as the scale and variance of the losses. We complement our theoretical results by demonstrating the effectiveness of our algorithm on synthetic benchmarks.

==> Defs/mathdefs.tex <==
%%Requeiried packages and preliminary definitions, needed by the options
\RequirePackage{mathtools}
% \RequirePackage{thmtools}
% \RequirePackage{amsfonts}
\RequirePackage{dsfont}
\RequirePackage{delimset}

%%Body of the package, most of the declarations appear here.

% Parenthethis
% \newcommand{\prn}[1]{\left( #1 \right)}
% \newcommand{\prn}[2][*]{\brk#1{#2}}
% \newcommand{\brc}[1]{\left\lbrace #1 \right\rbrace}
% \newcommand{\brc}[2][*]{\brk[c]#1{#2}}
% \newcommand{\brk}[1]{\left\lbrack #1 \right\rbrack}
% \newcommand{\abs}[1]{\left| #1 \right|}
% \newcommand{\underbracetxt}[2]{\underset{#2}{\underbrace{#1}}}

% Functions
% \newcommand{\norm}[1]{\left\lVert #1 \right\rVert}
% \newcommand{\innProd}[2]{\langle #1,#2 \rangle}
\newcommand{\innProd}[2][*]{\brk[a]#1{#2}}
\newcommand{\ceil}[2][*]{\delim\lceil\rceil#1{#2}}
\newcommand{\floor}[2][*]{\delim\lfloor\rfloor#1{#2}}
\newcommand{\indEvent}[2][*]{\mathds{1}_{\brk[c]#1{#2}}}
% \newcommand{\indEvent}[2][*]{\mathbb{1}{\brk[c]#1{#2}}}
\newcommand{\indFunc}[2][\infty]{\mathds{I}_{\brk[s]{#2,#1}}}
\newcommand{\indFuncAt}[3][\infty]{\indFunc[#1]{#2}\brk*{#3}}
\newcommand{\tr}[2][*]{\mathrm{Tr}\brk*{#2}}
\newcommand{\overbar}[1]{\mkern 2mu\overline{\mkern-2mu#1\mkern-2mu}\mkern 2mu}
\newcommand{\tran}{^{\mkern-1.5mu\mathsf{T}}}


% Standard Math Notations
\newcommand{\Oof}[2][*]{O\brk#1{#2}}
\newcommand{\OtildeOf}[2][*]{\smash{\widetilde{O}}\brk#1{#2}}
\newcommand{\EE}[1][]{\mathbb{E}_{#1}}
\newcommand{\EEBrk}[2][*]{\EE\delim{[}{]}#1{#2}}
\newcommand{\RR}[1][]{\mathbb{R}^{#1}}
\newcommand{\ZZ}[1][]{\mathbb{Z}^{#1}}
\newcommand{\NN}[1][]{\mathbb{N}^{#1}}
\newcommand{\ZZplus}[1][]{\mathbb{Z}^{#1}_{+}}
\newcommand{\PP}[2][*]{\mathbb{P}\brk#1{#2}}

\newcommand{\sphere}[1]{\mathcal{S}^{#1}}
\newcommand{\ball}[1]{\mathcal{B}^{#1}}

% Probability
\newcommand{\gaussDist}[2]{\mathcal{N}\brk0{#1, #2}}

% Math operators
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator*{\essinf}{ess\,inf}
\DeclareMathOperator*{\esssup}{ess\,sup}

% Definitions
\DeclarePairedDelimiterX\setDef[1]\lbrace\rbrace{\def\given{\;\delimsize\vert\;}#1}
\newcommand{\seqDef}[3]{\brk[c]*{#1}_{#2}^{#3}}

% General
\def\noi{\noindent}

\newcommand{\ifrac}[2]{#1/#2}
\newcommand{\minEigOf}[2][*]{\lambda_{\mathrm{min}}\brk#1{#2}}
\newcommand{\maxEigOf}[2][*]{\lambda_{\mathrm{max}}\brk#1{#2}}


\newcommand{\rootT}{\ensuremath{\smash{\sqrt{T}}}\xspace}
